CF-OPT: Counterfactual Explanations for Structured Prediction

Optimization layers in deep neural networks have enjoyed a growing popularity in structured learning, improving the state of the art on a variety of applications. Yet, these pipelines lack interpretability since they are made of two opaque layers: a highly non-linear prediction model, such as a deep neural network, and an optimization layer, which is typically a complex black-box solver. Our goal is to improve the transparency of such methods by providing counterfactual explanations. We build upon variational autoencoders a principled way of obtaining counterfactuals: working in the latent space leads to a natural notion of plausibility of explanations. We finally introduce a variant of the classic loss for VAE training that improves their performance in our specific structured context. These provide the foundations of CF-OPT, a first-order optimization algorithm that can find counterfactual explanations for a broad class of structured learning architectures. Our numerical results show that both close and plausible explanations can be obtained for problems from the recent literature.

==> algorithms/mdmm.tex <==
\begin{algorithm}[htb]
    \caption{Modified method of multipliers}
    \label{alg:mdmm}
    \begin{algorithmic}
        \STATE {\bfseries Initialize:} $k=0$, $x^0 = x_0$, $\lambda^0 = 0$, $\gamma >0$
        \WHILE{$x^k$ does not satisfy the explanation criterion}
        \STATE Update context: \text{$x^{k+1} \leftarrow x^k - \gamma \, \nabla_x \mathcal{E}(x^k, \lambda^k)$}
        \STATE Update Lagrange multiplier: \text{$\lambda^{k+1} \leftarrow \lambda^k + \gamma \, \nabla_\lambda \mathcal{E}(x^k, \lambda^k)$}
        \STATE $k \leftarrow k+1$
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}

==> figures/pipeline_as_equation.tex <==
\begin{equation}
    \label{eq:pipeline}
    \xrightarrow[]{\text{$x$}}
    \fbox{
        \begin{Bcenter}
            Predictor\\
            \textit{(k-NN or RF)}
        \end{Bcenter}}
    \xrightarrow[]{\text{$\{w_i(x)\}_{i=1}^n$}}
    \fbox{
        \begin{Bcenter}
            Optimization\\
            \textit{(Weighted SAA)}
        \end{Bcenter}}
    \xrightarrow[]{\text{$z^*$}}
\end{equation}
